Probing Late-type T dwarf J-H Color Outliers for Signs of Age

We present the results of a Keck/NIRSPEC follow-up survey of thirteen late-type T dwarfs (T6-T9), twelve of which have unusually red or blue J-H colors. Previous work suggests that J-H color outliers may represent the high-gravity, low-metallicity (old) and low-gravity, solar-metallicity (young) extremes of the late-type T dwarf population. We use medium-resolution Y- and H-band spectroscopy to probe regions of T dwarf atmospheres that are more sensitive to gravity and metallicity variations than the J band. We find that the spectral morphologies of our sample are largely homogeneous, with peak-normalized, Y- and H-band morphologies consistent with spectral standards. However, three objects stand out as potentially old, with overluminous Y-band spectra compared to their respective spectral standards, and a fourth object stands out as potentially young, with an underluminous Y band. Of these four objects, three have been previously identified as potential metallicity/gravity outliers, including the one object in our sample with a normal J-H color. We fit publicly available atmospheric model grids to our spectra and find that the best-fit physical parameters vary depending on the model used. As we continue to probe the characteristics of the late-T population, differences in synthetic spectra of ~10-20% in the blue wing of the Y band and ~45% at 1.65 microns, for the same physical parameters, must be reconciled. Further development and public availability of nonsolar metallicity models is also recommended. Future progress toward deciphering the impacts of gravity, metallicity, and variability in the late-type T dwarf population will also require high signal-to-noise, multiwavelength and multi-epoch photometry and spectroscopy.

==> obs_table_jhoutliers_update.tex <==
\begin{deluxetable}{cccccccccc}
\rotate
%\tablenum{1}
\label{table:observations}
\tablecolumns{10}
\tablecaption{NIRSPEC Observations}
\tabletypesize{\tiny}
\tablewidth{0in}
\tablehead{
\colhead{Object Name} &
\colhead{Short Name} &
\colhead{Discovery Ref.\tablenotemark{a}}&
\colhead{SpT}&
\colhead{SpT Ref.\tablenotemark{a}}&
\colhead{Band \tablenotemark{b}}&%,c}} &
\colhead{UT Date Observed}&
\colhead{Exp. Time (s)}&
\colhead{A0}&
\colhead{Slit Width (\asec)}
}

\startdata
WISE J000517.48+373720.5	&	WISE J0005+3737	&	1	&	T9	&	1	&	N1	&	2014 Nov 11	&	3600	&	HD 222749    	&	0.57	\\
	&		&	1	&	T9	&	1	&	N5	&	2014 Nov 11	&	3000	&	HD 222749    	&	0.57	\\
ULAS J013939.77+004813.8	&	ULAS J0139+0048	&	2	&	T7.5	&	2	&	N1	&	2014 Dec 2	&	4800	&	HD 18571 	&	0.57	\\
	&		&	2	&	T7.5	&	2	&	N5	&	2014 Dec 2	&	3600	&	HD 18571 	&	0.57	\\
CFBDS J030135.11-161418.0	&	CFBDS J0301-1614	&	3	&	T7p	&	3	&	N1	&	2014 Nov 11&	3600	&	HD 23683       	&	0.57	\\	
	&		&	3	&	T7p	&	3	&	N5	&	2014 Nov 12	&	4200	&	HD 23683       	&	0.57	\\
WISE J054047.00+483232.4	&	WISE J0540+4832	&	1	&	T8.5	&	1	&	N1	&	2014 Nov 11&	3000	&	HD 45105 	&	0.57	\\	
	&		&	1	&	T8.5	&	1	&	N5	&	2014 Nov 11	&	2400	&	HD 45105 	&	0.57	\\
WISE J075946.98-490454.0	&	WISE J0759-4904	&	4	&	T8	&	4	&	N1	&	2014 Dec 2	&	4200	&	HD 74042	&	0.57	\\
CFBDS J092250.12+152741.4	&	CFBDS J0922+1527	&	3	&	T7	&	3	&	N1	&	2014 Apr 14	&	3600	&	HD 111744 	&	0.57	\\
	&		&	3	&	T7	&	3	&	N5	&	2014 Dec 3	&	3000	&	HD 79108	&	0.57	\\
ULAS J095047.28+011734.3	&	ULAS J0950+0117	&	5	&	T8p	&	5	&	N1	&	2014 Apr 13	&	3600	&	HD 95126	&	0.57	\\
	&		&	5	&	T8p	&	5	&	N5	&	2014 Dec 2	&	3000	&	HD 79108	&	0.57	\\
ULAS J101721.40+011817.9	&	ULAS J1017+0118	&	6	&	T8p	&	6	&	N5	&	2014 Dec 3	&	3000	&	HD 79108	&	0.57	\\
ULAS J150457.65+053800.8	&	HIP 73786B	&	7	&	T6p	&	8	&	N1	&	2014 Apr 14	&	1800	&	7 Ser	&	0.57	\\
	&		&	7	&	T6p	&	8	&	N5	&	2014 Jun 20	&	2400	&	 HD 123233	&	0.57	\\
WISE J161441.46+173935.5	&	WISE J1614+1739	&	4	&	T9	&	4	&	N1	&	2014 Apr 13	&	2400	&	26 Ser	&	0.57	\\
	&		&	4	&	T9	&	4	&	N1	&	2014 Apr 14	&	2400	&	26 Ser	&	0.57	\\
WISE J161705.74+180714.1	&	WISE J1617+1807	&	9	&	T8	&	9	&	N1	&	2014 Apr 12	&	2400	&	q Her	&	0.57	\\
	&		&	9	&	T8	&	9	&	N5	&	2014 Jun 20 &	2400	&	q Her	&	0.57	\\	
WISE J181210.85+272144.3	&	WISE J1812+2721	&	9	&	T8.5	&	9	&	N1	&	2014 Jun 21	&	1800	&	HD 199217	&	0.57	\\
	&		&	9	&	T8.5	&	9	&	N5	&	2014 Jun 20	&	2400	&	HD 192538 	&	0.57	\\
ULAS J214638.83-001038.7	&	Wolf 940B	&	10	&	T8.5	&	10	&	N1	&	2014 Jun 21	&	2400	&	HD 210501	&	0.57	\\
	&		&	10	&	T8.5	&	10	&	N5	&	2014 Nov 11	&	2400	&	HD 210501	&	0.57	\\
\cutinhead{Previously Unpublished NIRSPEC Spectral Standard Observations}																			
2MASSI J0415195-093506	&	2MASS J0415-0935	&	11	&	T8	&	12	&	N1	&	2002 Dec 23	&	1200	&	HD 34481	&	0.38	\\
UGPS J072227.51-054031.2	&	UGPS J0722-0540	&	13	&	T9	&	14	&	N1	&	2014 Dec 2	&	1800	&	HD 64653	&	0.57	\\
	&		&	13	&	T9	&	14	&	N5	&	2014 Dec 3	&	1800	&	HD 64653	&	0.57	\\
2MASSI J0727182+171001	&	2MASS J0727+1710	&	11	&	T7	&	12	&	N1	&	2014 Nov 12 &	1800	&	HD 57208	&	0.57	\\	
	&		&	11	&	T7	&	12	&	N5	&	2014 Nov 12	&	1800	&	HD 57208	&	0.57	\\
\cutinhead{Previously Unpublished Brown Dwarf Spectroscopic Survey (BDSS; \citealt{McLean2003}) Comparison Object Observation}																			
2MASSI J0937347+293142	&	2MASS J0937+2931	&	11	&	T6p	&	12	&	N1	&	2001 Mar 7 &	1200 &	AG +27 1006 &	  0.38\\				
\enddata
